Understanding Expectations for a Robotic Guide Dog for Visually Impaired People

Robotic guide dogs hold significant potential to enhance the autonomy and mobility of blind or visually impaired (BVI) individuals by offering universal assistance over unstructured terrains at affordable costs. However, the design of robotic guide dogs remains underexplored, particularly in systematic aspects such as gait controllers, navigation behaviors, interaction methods, and verbal explanations. Our study addresses this gap by conducting user studies with 18 BVI participants, comprising 15 cane users and three guide dog users. Participants interacted with a quadrupedal robot and provided both quantitative and qualitative feedback. Our study revealed several design implications, such as a preference for a learning-based controller and a rigid handle, gradual turns with asymmetric speeds, semantic communication methods, and explainability. The study also highlighted the importance of customization to support users with diverse backgrounds and preferences, along with practical concerns such as battery life, maintenance, and weather issues. These findings offer valuable insights and design implications for future research and development of robotic guide dogs.

==> table/bvi-info.tex <==
% \begin{table}[t]
\begin{table*}[t]
    \centering
    % \setlength\tabcolsep{1pt}
    \begin{tabular}{cccccc}
    % \hline
    \toprule
        \textbf{ID} & \textbf{Age} & \textbf{Gender} & \textbf{Impairment Condition} & \textbf{Mobility Aid}\\ \midrule
        P01 & 67 & Male & Low vision, some light perception & White Cane\\
        P02 & 64 & Male & No sight in right, low vision in left & White Cane\\
        P03 & 56 & Male & Low vision & Guide Dog\\
        P04 & 64 & Female & Blind & White Cane\\
        P05 & 51 & Female & No sight in right, low vision in left 
        % (Glaucoma, Diabetic sight)
        & White Cane\\ \addlinespace
        P06 & 77 & Male & Blind & White Cane\\
        P07 & 51 & Female & Blind & White Cane\\
        P08 & 68 & Female & {Low vision, some light perception; hearing impaired} & White Cane\\
        % P08 & 68 & Female & \textls[-1]{Low vision, light perception; hearing impaired} & White Cane\\
        P09 & 67 & Male & {Low vision, low depth perception; hearing impaired} & White Cane\\
        % P09 & 67 & Male & \textls[-50]{Low vision, low depth perception; hearing impaired} & White Cane\\
        % P09 & 67 & Male & \scalebox{.9}[1.0]{Low vision, low depth perception; hearing loss} & White Cane\\
        P10 & 51 & Male & Blind & White Cane\\
        % P10 & 51 & Male & Blind (Diabetic Retinopothy) & White Cane\\
        \addlinespace
        P11 & 37 & Female & Low vision & White Cane\\
        % P11 & 37 & Female & Low vision (Uveitis, Retinal detachment) & White Cane\\
        P12 & 64 & Female & Low vision, only light perception & White Cane\\
        P13 & 34 & Female & Low vision, no depth perception, low color perception & White Cane\\
        P14 & 69 & Male & Blind & Guide Dog\\
        P15 & 68 & Female & Low vision, somewhat light/depth perception & White Cane\\ \addlinespace
        P16 & 62 & Female & No sight in left, low vision in right; hearing impaired & Guide Dog\\
        P17 & 66 & Female & Low vision, no color/depth perception; hearing impaired & White Cane\\
        P18 & 46 & Male & Low vision & White Cane\\
        \bottomrule
    \end{tabular}
    \caption{Demographic information of the BVI participants}
    \label{tab:bvi-info}
% \end{table}
\end{table*}
